Transformaly -- Two (Feature Spaces) Are Better Than One

Anomaly detection is a well-established research area that seeks to identify samples outside of a predetermined distribution. An anomaly detection pipeline is comprised of two main stages: (1) feature extraction and (2) normality score assignment. Recent papers used pre-trained networks for feature extraction achieving state-of-the-art results. However, the use of pre-trained networks does not fully-utilize the normal samples that are available at train time. This paper suggests taking advantage of this information by using teacher-student training. In our setting, a pretrained teacher network is used to train a student network on the normal training samples. Since the student network is trained only on normal samples, it is expected to deviate from the teacher network in abnormal cases. This difference can serve as a complementary representation to the pre-trained feature vector. Our method -- Transformaly -- exploits a pre-trained Vision Transformer (ViT) to extract both feature vectors: the pre-trained (agnostic) features and the teacher-student (fine-tuned) features. We report state-of-the-art AUROC results in both the common unimodal setting, where one class is considered normal and the rest are considered abnormal, and the multimodal setting, where all classes but one are considered normal, and just one class is considered abnormal. The code is available at https://github.com/MatanCohen1/Transformaly.

==> latex/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> latex/problem_statement.tex <==
\paragraph{Problem Statement}
In this paper, we examine two variants of the semantic anomaly detection tasks in images: the unimodal and the multimodal settings. Unimodal settings refer to the paradigm commonly used in the research community to simulate semantic anomaly detection. As the source of natural images, a well-known dataset, such as cifar10 or cifar100, is used. One semantic class is randomly chosen as normal while the rest of the classes are treated as abnormal. During training, the model is exposed just to the normal class’ samples. In inference time, all samples of the test set are evaluated, while samples that are not from the normal class are considered anomalous. 

We claim that this does not fully capture the challenges associated with detecting semantic anomalies. First, in real-life scenarios, it is common that the normal data has various forms, such as several different semantic classes or behaviors, and taking just one class as normal simplifies the problem and ignores its complex nature. In addition, following this paradigm leads to a peculiar evaluation process, where we have much more anomalies than normal samples (nine and nineteen times more for cifar10 and cifar100 respectively). This is not in line with a common anomaly detection use case where the normal samples are the majority of the data the model encounters and the anomalies are the rare events. Moreover, it can damage the evaluation process and misrepresent the model’s real performance. As an example, consider the twenty-class cifar100 dataset, which was evaluated in a unimodal setting. Using this setting, the evaluation process contains 500 normal samples and 9,500 abnormal samples. Suppose we suggested a model that confuses the normal class samples with samples of one of the abnormal classes. The samples’ scores of these two classes will be higher than all other samples, indicating that the model considers both of them normal. In spite of its low precision getting by setting any threshold, this model's AUROC score is likely to be high because of the large number of anomalies in the evaluation process, as can be shown in figure x. As a result, we can be led to believe this model is performing well. One can argue that adding a precision score to our evaluation process is the solution to this problem. Although it can reveal this delicate situation, it will force us to set a threshold in order to hard-classify samples, and it does not address the previously mentioned problems. This misleading phenomenon has been demonstrated in previous state-of-the-art solutions, as detailed in section 5.1. Furthermore, this unimodal setting is saturated, with an AUROC score of around 98\%. In light of the fact that these datasets contain mislabeled samples, as discussed in section 5.3.1, and dark images, which are almost impossible to classify, discussed in section 5.3.2, we can assume that near-perfect results have already been achieved. As a result, the motivation to keep beating the current state-of-the-art results is questionable, and it casts a shadow over whether we are indeed improving our solutions, or simply overfitting them to these datasets. In the light of the above statements, should we keep evaluate our solutions using just one class as normal?.

Researchers have emerged with an inadequate paradigm not only for anomaly detection but also for OOD detection. The common benchmark in the OOD detection domain is to use one dataset for the multiclass classification task, and a second dataset for the evaluation of the OOD detector. Courville and Ahmed recently criticized this benchmark, claiming that it is ill-motivated and the OOD detection can be explained by low-level image statistics, or by underlying biases of the two datasets \cite{ahmed2020detecting}. While discussing other problems in the OOD domain, which we leave for further reading, the authors suggest using a single dataset for both the multiclass classification task and the OOD detection. Their solution is to treat one class as an out-distribution and all other classes as in-distributions, which will be used for classification. We extend their proposed paradigm for anomaly detection as complementary to the regular unimodal setting, evaluating the current approaches extensively. In this setting, we treat all classes as normal but one, which we treat as abnormal. During the training process, we do not use the labels of the normal samples but simply treat them as a single multimodal normal class. We believe that the two settings are necessary in order to fully evaluate any anomaly detection solution.

All of the mentioned solutions are applied on the regular unimodal settings, except two which reported their results also on the multimodal settings: GANnomaly and DN2 \cite{akcay2018ganomaly, reiss2020panda}. GANomaly is a conditional generative adversarial network that jointly learns the generation of high-dimensional image space and the inference of latent space \cite{akcay2018ganomaly}. The architecture is composed of encoder-decoder-encoder sub-networks and used a distance between the original image’s representation and the reconstructed image’s representation as an anomaly score. As mentioned before DN2 uses an imagenet pretrained resent model as a feature extractor that produces samples' representation. Based on these normal training data representations, they determine the distance a test sample has to its k nearest neighbor as an anomaly score. These papers reported their performance in the multimodal setting briefly and did not perform an extensive evaluation and comprehensive comparison with other methods as we did.

==> latex/tables/diagonal_full_ablation.tex <==
\begin{table}[]
\small
\centering
\begin{tabular}{|l|l|l|}
\hline
Dataset    & 
\multicolumn{1}{c|}{\thead{Full Covariance}} & 
\multicolumn{1}{c|}{Diagonal Covariance} \\
\hline
CIFAR10    &
\multicolumn{1}{c|}{98.31} &
\multicolumn{1}{c|}{\textbf{98.36}} \\
\cline{1-1}
CIFAR100   &
\multicolumn{1}{c|}{97.34} &
\multicolumn{1}{c|}{\textbf{97.70}} \\
\cline{1-1}
FMNIST     & 
\multicolumn{1}{c|}{\textbf{94.43}} &
\multicolumn{1}{c|}{94.38} \\
\cline{1-1}
CatsVsDogs     & 
\multicolumn{1}{c|}{\textbf{99.52}} &
\multicolumn{1}{c|}{99.45} \\
\cline{1-1}
DIOR     & 
\multicolumn{1}{c|}{98.08} &
\multicolumn{1}{c|}{\textbf{98.47}} \\
\cline{1-1}
Blood Cells     & 
\multicolumn{1}{c|}{\textbf{74.85}} &
\multicolumn{1}{c|}{74.59} \\
\cline{1-1}
Covid19     & 
\multicolumn{1}{c|}{98.87} &
\multicolumn{1}{c|}{\textbf{99.26}} \\
\cline{1-1}
Weather     & 
\multicolumn{1}{c|}{94.32} &
\multicolumn{1}{c|}{\textbf{95.35}} \\
\cline{1-1}
View     & 
\multicolumn{1}{c|}{\textbf{95.80}} &
\multicolumn{1}{c|}{95.96} \\
\cline{1-1}
Concrete     &
\multicolumn{1}{c|}{\textbf{99.77}} &
\multicolumn{1}{c|}{\textbf{99.77}} \\
\cline{1-1}
\hline
\end{tabular}
\caption{{\bf AUROC score of the Unimodal setting:} Comparison between diagonal and full covariance matrix.}
\label{table:diagonal_full_ablation}
\end{table}



==> latex/tables/dino_comparison_rebuttal.tex <==



\begin{table}[]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Dataset    &
\multicolumn{1}{l|}{CIFAR10} &
\multicolumn{1}{l|}{CIFAR100} &
\multicolumn{1}{l|}{FMNIST} &
\multicolumn{1}{l|}{CatsDogs} &
\multicolumn{1}{l|}{DIOR}\\
\hline
DINO    &
\multicolumn{1}{c|}{97.25} &
\multicolumn{1}{c|}{97.07} &
\multicolumn{1}{c|}{\textbf{94.62}} &
\multicolumn{1}{c|}{97.33} &
\multicolumn{1}{c|}{97.81} \cr 
% \cline{1-1}
\hline
Ours   &
\multicolumn{1}{c|}{\textbf{98.31}} &
\multicolumn{1}{c|}{\textbf{97.34}} &
\multicolumn{1}{c|}{94.43} &
\multicolumn{1}{c|}{\textbf{99.52}} &
\multicolumn{1}{c|}{\textbf{98.08}} \cr 
\hline
\end{tabular}
\caption{{\bf AUROC scores of the unimodal setting:} We compare our method against DINO using Gaussian as scoring method. Scores taken from submission.}
\label{table:dino_comparison_rebuttal}
\end{table}


==> latex/tables/knn_gm_ablation_multimodal.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
Dataset    &
\multicolumn{1}{l|}{\thead{$k$-NN \\ $k=2$ }} &
\multicolumn{1}{l|}{\thead{$k$-NN \\ $k=5$ }} &
\multicolumn{1}{l|}{\thead{$k$-NN \\ $k=10$ }} &
\multicolumn{1}{l|}{\thead{GMM \\ $n=1$ }} &
\multicolumn{1}{l|}{\thead{GMM \\ $n=5$ }} &
\multicolumn{1}{l|}{\thead{GMM \\ $n=10$ }} &
\multicolumn{1}{l|}{\thead{GMM \\ $n=20$ }} \\
\hline
CIFAR10    &
\multicolumn{1}{|c|}{88.76} &
\multicolumn{1}{c|}{89.16} &
\multicolumn{1}{c|}{89.40} &
\multicolumn{1}{c|}{90.23} &
\multicolumn{1}{c|}{\textbf{90.81}} &
\multicolumn{1}{c|}{\underline{90.56}} &
\multicolumn{1}{c|}{90.39} \cr 
\cline{1-1}
CIFAR100   &
\multicolumn{1}{|c|}{82.20} &
\multicolumn{1}{c|}{\underline{82.68}} &
\multicolumn{1}{c|}{\textbf{82.87}} &
\multicolumn{1}{c|}{78.76} &
\multicolumn{1}{c|}{79.42} &
\multicolumn{1}{c|}{78.99} &
\multicolumn{1}{c|}{77.66} \cr 
\cline{1-1}
FMNIST     &
\multicolumn{1}{|c|}{75.59} &
\multicolumn{1}{c|}{74.99} &
\multicolumn{1}{c|}{74.51} &
\multicolumn{1}{c|}{72.29} &
\multicolumn{1}{c|}{75.43} &
\multicolumn{1}{c|}{\underline{76.92}} &
\multicolumn{1}{c|}{\textbf{78.00}} \cr 
\cline{1-1}
DIOR &
\multicolumn{1}{|c|}{66.66} &
\multicolumn{1}{c|}{66.08} &
\multicolumn{1}{c|}{65.73} &
\multicolumn{1}{c|}{65.72} &
\multicolumn{1}{c|}{69.75} &
\multicolumn{1}{c|}{\textbf{70.21}} &
\multicolumn{1}{c|}{\underline{69.82}} \cr 
\hline
\end{tabular}
\caption{{\bf Modeling functions in the multimodal setting:} We report AUROC results of our algorithm using different modelling functions on the pre-trained features. In particular, we try $k$-NN with different values of $k$, the number of nearest neighbors. We also test Gaussian Mixture Model (GMM) with varying number of Gaussians. It can be observed that no modelling function is consistently better than the others. This leads us to use a single Gaussian ("GMM, $n=1$" in the table) because if offers an attractive trade-off between high accuracy, low memory footprint and fast compute time. 
}
\label{table:multimodal_knn_gm_ablation}
\end{table*}




==> latex/tables/knn_gm_ablation_unimodal.tex <==

\begin{table*}[]
\small
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
Dataset    &
\multicolumn{1}{l|}{\thead{$k$-NN \\ $k=2$ }} &
\multicolumn{1}{l|}{\thead{$k$-NN \\ $k=5$ }} &
\multicolumn{1}{l|}{\thead{$k$-NN \\ $k=10$ }} &
\multicolumn{1}{l|}{\thead{GMM \\ $n=1$ }} &
\multicolumn{1}{l|}{\thead{GMM \\ $n=5$ }} &
\multicolumn{1}{l|}{\thead{GMM \\ $n=10$ }} &
\multicolumn{1}{l|}{\thead{GMM \\ $n=20$ }} \\
\hline
CIFAR10    &
\multicolumn{1}{|c|}{\underline{97.81}} &
\multicolumn{1}{c|}{\textbf{97.84}} &
\multicolumn{1}{c|}{\underline{97.81}} &
\multicolumn{1}{c|}{\underline{97.81}} &
\multicolumn{1}{c|}{97.79} &
\multicolumn{1}{c|}{96.20} &
\multicolumn{1}{c|}{95.98} \cr 
\cline{1-1}
CIFAR100   &
\multicolumn{1}{|c|}{\textbf{96.41}} &
\multicolumn{1}{c|}{\underline{96.40}} &
\multicolumn{1}{c|}{96.33} &
\multicolumn{1}{c|}{96.25} &
\multicolumn{1}{c|}{95.18} &
\multicolumn{1}{c|}{92.42} &
\multicolumn{1}{c|}{91.00} \cr 
\cline{1-1}
FMNIST     &
\multicolumn{1}{|c|}{\textbf{94.19}} &
\multicolumn{1}{c|}{\underline{94.09}} &
\multicolumn{1}{c|}{94.00} &
\multicolumn{1}{c|}{93.94} &
\multicolumn{1}{c|}{93.69} &
\multicolumn{1}{c|}{94.06} &
\multicolumn{1}{c|}{93.04} \cr 
\cline{1-1}
CatsVsDogs &
\multicolumn{1}{|c|}{99.59} &
\multicolumn{1}{c|}{\textbf{99.63}} &
\multicolumn{1}{c|}{\textbf{99.63}} &
\multicolumn{1}{c|}{\underline{99.60}} &
\multicolumn{1}{c|}{\textbf{99.63}} &
\multicolumn{1}{c|}{98.67} &
\multicolumn{1}{c|}{98.97} \cr
\cline{1-1}
DIOR &
\multicolumn{1}{|c|}{91.74} &
\multicolumn{1}{c|}{92.52} &
\multicolumn{1}{c|}{\underline{93.03}} &
\multicolumn{1}{c|}{\textbf{93.97}} &
\multicolumn{1}{c|}{91.27} &
\multicolumn{1}{c|}{88.68} &
\multicolumn{1}{c|}{88.78} \cr 
\hline
\end{tabular}
\caption{{\bf Modeling functions in the unimodal setting:} We report AUROC results of our algorithm using different modelling functions on the pre-trained features only. In particular, we try $k$-NN with different values of $k$, the number of nearest neighbors. We also test Gaussian Mixture Model (GMM) with varying number of Gaussians. It can be observed that no modelling function is consistently better than the others. This leads us to use a single Gaussian ("GMM, $n=1$" in the table) because if offers an attractive trade-off between high accuracy, low memory footprint and fast compute time.
}
\label{table:unimodal_knn_gm_ablation}
\end{table*}





% \begin{table*}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% Dataset    &
% \multicolumn{1}{l|}{$k$-NN, k=2} &
% \multicolumn{1}{l|}{$k$-NN, k=5} &
% \multicolumn{1}{l|}{$k$-NN, k=10} &
% \multicolumn{1}{l|}{GM, n = 1} &
% \multicolumn{1}{l|}{GM, n = 5} &
% \multicolumn{1}{l|}{GM, n = 10} &
% \multicolumn{1}{l|}{GM, n = 20} \\
% \hline
% CIFAR10    &
% \multicolumn{1}{|c|}{97.74} &
% \multicolumn{1}{c|}{98.01} &
% \multicolumn{1}{c|}{\underline{98.13}} &
% \multicolumn{1}{c|}{\textbf{98.16}} &
% \multicolumn{1}{c|}{97.31} &
% \multicolumn{1}{c|}{95.60} &
% \multicolumn{1}{c|}{97.53} \cr 
% \cline{1-1}
% CIFAR100   &
% \multicolumn{1}{|c|}{96.96} &
% \multicolumn{1}{c|}{97.26} &
% \multicolumn{1}{c|}{\textbf{97.41}} &
% \multicolumn{1}{c|}{\underline{97.48}} &
% \multicolumn{1}{c|}{92.23***} &
% \multicolumn{1}{c|}{96.30***} &
% \multicolumn{1}{c|}{96.92***} \cr 
% \cline{1-1}
% FMNIST     &
% \multicolumn{1}{|c|}{94.18} &
% \multicolumn{1}{c|}{94.12} &
% \multicolumn{1}{c|}{94.03} &
% \multicolumn{1}{c|}{\textbf{94.76}} &
% \multicolumn{1}{c|}{\underline{94.40}} &
% \multicolumn{1}{c|}{92.12} &
% \multicolumn{1}{c|}{92.80} \cr 
% \cline{1-1}
% CatsVsDogs &
% \multicolumn{1}{|c|}{99.32} &
% \multicolumn{1}{c|}{\textbf{99.57}} &
% \multicolumn{1}{c|}{\underline{99.58}} &
% \multicolumn{1}{c|}{99.03} &
% \multicolumn{1}{c|}{98.44} &
% \multicolumn{1}{c|}{99.02} &
% \multicolumn{1}{c|}{94.97} \cr
% \cline{1-1}
% DIOR &
% \multicolumn{1}{|c|}{91.93} &
% \multicolumn{1}{c|}{92.20} &
% \multicolumn{1}{c|}{92.40} &
% \multicolumn{1}{c|}{\textbf{93.94}} &
% \multicolumn{1}{c|}{92.69} &
% \multicolumn{1}{c|}{\underline{93.17}} &
% \multicolumn{1}{c|}{92.71} \cr 
% \hline
% \end{tabular}
% \caption{{\bf AUROC scores of the unimodal setting using different K and number of components for $k$-NN and Gaussian Mixture Model.}
% }
% \label{table:unimodal_knn_gm_ablation}
% \end{table*}




==> latex/tables/knn_gmm_ablations.tex <==
\begin{table*}
\parbox{.45\linewidth}{
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Dataset    &
\multicolumn{1}{l|}{\thead{$k$-NN \\ $k=2$ }} &
\multicolumn{1}{l|}{\thead{$k$-NN \\ $k=5$ }} &
% \multicolumn{1}{l|}{\thead{$k$-NN \\ $k=10$ }} &
\multicolumn{1}{l|}{\thead{GMM \\ $n=1$ }} &
\multicolumn{1}{l|}{\thead{GMM \\ $n=5$ }} &
% \multicolumn{1}{l|}{\thead{GMM \\ $n=10$ }} &
\multicolumn{1}{l|}{\thead{GMM \\ $n=20$ }} \\
\hline
CIFAR10    &
\multicolumn{1}{|c|}{\underline{97.81}} &
\multicolumn{1}{c|}{\textbf{97.84}} &
% \multicolumn{1}{c|}{\underline{97.81}} &
\multicolumn{1}{c|}{\underline{97.81}} &
\multicolumn{1}{c|}{97.79} &
% \multicolumn{1}{c|}{96.20} &
\multicolumn{1}{c|}{95.98} \cr 
\cline{1-1}
CIFAR100   &
\multicolumn{1}{|c|}{\textbf{96.41}} &
\multicolumn{1}{c|}{\underline{96.40}} &
% \multicolumn{1}{c|}{96.33} &
\multicolumn{1}{c|}{96.25} &
\multicolumn{1}{c|}{95.18} &
% \multicolumn{1}{c|}{92.42} &
\multicolumn{1}{c|}{91.00} \cr 
\cline{1-1}
FMNIST     &
\multicolumn{1}{|c|}{\textbf{94.19}} &
\multicolumn{1}{c|}{\underline{94.09}} &
% \multicolumn{1}{c|}{94.00} &
\multicolumn{1}{c|}{93.94} &
\multicolumn{1}{c|}{93.69} &
% \multicolumn{1}{c|}{94.06} &
\multicolumn{1}{c|}{93.04} \cr 
\cline{1-1}
CatsVsDogs &
\multicolumn{1}{|c|}{99.59} &
\multicolumn{1}{c|}{\textbf{99.63}} &
% \multicolumn{1}{c|}{\textbf{99.63}} &
\multicolumn{1}{c|}{\underline{99.60}} &
\multicolumn{1}{c|}{\textbf{99.63}} &
% \multicolumn{1}{c|}{98.67} &
\multicolumn{1}{c|}{98.97} \cr
\cline{1-1}
DIOR &
\multicolumn{1}{|c|}{91.74} &
\multicolumn{1}{c|}{\underline{92.52}} &
% \multicolumn{1}{c|}{\underline{93.03}} &
\multicolumn{1}{c|}{\textbf{93.97}} &
\multicolumn{1}{c|}{91.27} &
% \multicolumn{1}{c|}{88.68} &
\multicolumn{1}{c|}{88.78} \cr 
\hline
\end{tabular}
\caption{{\bf Modeling functions in the unimodal setting}}
\label{table:reduced_unimodal_knn_gm_ablation_comb}
% \end{subtable}
}
\hfill
\parbox{.45\linewidth}{
\centering
% \begin{subtable}[]{0.3\textwidth}
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Dataset    &
\multicolumn{1}{l|}{\thead{$k$-NN \\ $k=2$ }} &
\multicolumn{1}{l|}{\thead{$k$-NN \\ $k=5$ }} &
% \multicolumn{1}{l|}{\thead{$k$-NN \\ $k=10$ }} &
\multicolumn{1}{l|}{\thead{GMM \\ $n=1$ }} &
\multicolumn{1}{l|}{\thead{GMM \\ $n=5$ }} &
% \multicolumn{1}{l|}{\thead{GMM \\ $n=10$ }} &
\multicolumn{1}{l|}{\thead{GMM \\ $n=20$ }} \\
\hline
CIFAR10    &
\multicolumn{1}{|c|}{88.76} &
\multicolumn{1}{c|}{89.16} &
% \multicolumn{1}{c|}{89.40} &
\multicolumn{1}{c|}{90.23} &
\multicolumn{1}{c|}{\textbf{90.81}} &
% \multicolumn{1}{c|}{\underline{90.56}} &
\multicolumn{1}{c|}{\underline{90.39}} \cr 
\cline{1-1}
CIFAR100   &
\multicolumn{1}{|c|}{\underline{82.20}} &
\multicolumn{1}{c|}{\textbf{82.68}} &
% \multicolumn{1}{c|}{\textbf{82.87}} &
\multicolumn{1}{c|}{78.76} &
\multicolumn{1}{c|}{79.42} &
% \multicolumn{1}{c|}{78.99} &
\multicolumn{1}{c|}{77.66} \cr 
\cline{1-1}
FMNIST     &
\multicolumn{1}{|c|}{\underline{75.59}} &
\multicolumn{1}{c|}{74.99} &
% \multicolumn{1}{c|}{74.51} &
\multicolumn{1}{c|}{72.29} &
\multicolumn{1}{c|}{75.43} &
% \multicolumn{1}{c|}{\underline{76.92}} &
\multicolumn{1}{c|}{\textbf{78.00}} \cr 
\cline{1-1}
DIOR &
\multicolumn{1}{|c|}{66.66} &
\multicolumn{1}{c|}{66.08} &
% \multicolumn{1}{c|}{65.73} &
\multicolumn{1}{c|}{65.72} &
\multicolumn{1}{c|}{\underline{69.75}} &
% \multicolumn{1}{c|}{\textbf{70.21}} &
\multicolumn{1}{c|}{\textbf{69.82}} \cr 
\hline
\end{tabular}
\caption{{\bf Modeling functions in the multimodal setting} 
% \matan{1. This is a copy of the description of Table 4. Maybe we should merge them? 2. Shir's comment:"GMM, N=1 is not the best in any category and even the worst on two of the four datasets. Im semsomg this could be problematic.". She's got a point...}
}
\label{table:reduced_multimodal_knn_gm_ablation_comb}
}

\caption{We report AUROC results of our algorithm using different modelling functions on the pre-trained features. In particular, we try $k$-NN with different values of $k$, the number of nearest neighbors. We also test Gaussian Mixture Model (GMM) with varying number of Gaussians. It can be observed that no modelling function is consistently better than the others. This leads us to use a single Gaussian ("GMM, $n=1$" in the table) because if offers an attractive trade-off between high accuracy, low memory footprint and fast compute time.}
\end{table*}

% \begin{table*}
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{ccc}
% \hline
% a&b&c\\
% \hline
% \end{tabular}
% \caption{Foo}
% }
% \hfill
% \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{ccc}
% \hline
% d&e&f\\
% \hline
% \end{tabular}
% \caption{Bar}
% }
% \end{table*}

==> latex/tables/multimodal_ablation.tex <==
\begin{table*}[h!]
\centering
\begin{tabular*}{\textwidth}{@{\extracolsep{\stretch{1}}}*{11}{r}@{}}
\hline
Dataset  & \multicolumn{1}{l|}{GM} & 
\multicolumn{1}{p{2cm}|}{\centering {BOP of the \newline last block}} & \multicolumn{1}{p{2cm}|}{\centering {BOP of the \newlinethree last blocks}} &
\multicolumn{1}{p{2cm}|}{\centering {BOP of the \newline ten last blocks}} &
\multicolumn{1}{p{2cm}|}{\centering {GM + BOP of \newline the  last block}} &
\multicolumn{1}{p{2cm}|}{\centering {GM + BOP of \newline the  three last blocks}} &
\multicolumn{1}{p{2cm}}{\centering {GM +BOP of \newline  the ten last block}} \\
\hline
CIFAR10    &
\multicolumn{1}{c|}{87.58} &
\multicolumn{1}{c|}{87.79} & \multicolumn{1}{c|}{88.66} &
\multicolumn{1}{c|}{80.15} &
\multicolumn{1}{c|}{91.74} &
\multicolumn{1}{c|}{90.24} &
\multicolumn{1}{c}{85.39} \\
\cline{1-1}
CIFAR100   &
\multicolumn{1}{c|}{80.41} &
\multicolumn{1}{c|}{71.35} &
\multicolumn{1}{c|}{78.19} &
\multicolumn{1}{c|}{ 75.46} &
\multicolumn{1}{c|}{85.06} &
\multicolumn{1}{c|}{83.05} &
\multicolumn{1}{c}{79.15} &
\\ 
\cline{1-1}
FMNIST     &
\multicolumn{1}{c|}{74.83} &
\multicolumn{1}{c|}{70.51} &
\multicolumn{1}{c|}{71.60} &
\multicolumn{1}{c|}{72.26} &
\multicolumn{1}{c|}{75.04} &
\multicolumn{1}{c|}{\textbf{73.90}} &
\multicolumn{1}{c}{73.77} &
\\
\cline{1-1}
DIOR &
\multicolumn{1}{c|}{58.68} &
\multicolumn{1}{c|}{61.22} &
\multicolumn{1}{c|}{59.50} &
\multicolumn{1}{c|}{64.84} &
\multicolumn{1}{c|}{60.21} &
\multicolumn{1}{c|}{59.83} &
\multicolumn{1}{c}{\textbf{63.91}} &
\\ 
\hline
\end{tabular*}
\caption{{\bf AUROC score of the multimodal setting} Our method ranks first on cifar10 and cifar100, and second on FMNIST. See text for discussion about the DIOR dataset.}
\label{table:multimodal-aux}
\end{table*}


==> latex/tables/multimodal_transposed.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
Dataset  &
\multicolumn{1}{c|}{CIFAR10} &
\multicolumn{1}{c|}{CIFAR100} &
\multicolumn{1}{c|}{FMNIST} &
\multicolumn{1}{c|}{DIOR} \\
\hline
DeepSVDD   &
\multicolumn{1}{c|}{50.67} &
\multicolumn{1}{c|}{50.75} &
\multicolumn{1}{c|}{-} &
\multicolumn{1}{c|}{-} &
\cline{1-1}

CSI &
\multicolumn{1}{c|}{-} &
\multicolumn{1}{c|}{-} &
\multicolumn{1}{c|}{-} &
\multicolumn{1}{c|}{-} &
\cline{1-1}
DN2 &
\multicolumn{1}{c|}{71.7} &
\multicolumn{1}{c|}{71.0} &
\multicolumn{1}{c|}{-} &
\multicolumn{1}{c|}{\underline{68.08*}} & 
\cline{1-1}
PANDA &
\multicolumn{1}{c|}{68.51} &
\multicolumn{1}{c|}{62.47} &
\multicolumn{1}{c|}{\textbf{79.45}} &
\multicolumn{1}{c|}{-} &
\cline{1-1}
MSAD &
\multicolumn{1}{c|}{71.52} &
\multicolumn{1}{c|}{67.65} &
\multicolumn{1}{c|}{72.26} &
\multicolumn{1}{c|}{\textbf{75.03*}} &
\cline{1-1}
GM &
\multicolumn{1}{c|}{87.58} &
\multicolumn{1}{c|}{\underline{80.41}} &
\multicolumn{1}{c|}{\underline{74.83}} &
\multicolumn{1}{c|}{56.68} &
\cline{1-1}
BoP &
\multicolumn{1}{c|}{\underline{88.66}} &
\multicolumn{1}{c|}{78.19} &
\multicolumn{1}{c|}{71.60} &
\multicolumn{1}{c|}{59.50} &
\cline{1-1}
GM+BoP &
\multicolumn{1}{c|}{\textbf{90.24}} &
\multicolumn{1}{c|}{\textbf{83.05}} &
\multicolumn{1}{c|}{73.90} &
\multicolumn{1}{c|}{59.83} &
\hline
\end{tabular}
\caption{{\bf AUROC scores of the unimodal setting.} We compare our three variants of our method (BoP only, GM only, and GM+BoP) against the alternative. We outperform all methods on both cifar10 and cifar100, and come in second on both the CatsVsDogs and FMNIST datasets.}
\label{table:unimodal}
\end{table}


==> latex/tables/unimodal_ablation.tex <==
\begin{table*}[h!]
\centering
\begin{tabular*}{\textwidth}{@{\extracolsep{\stretch{1}}}*{11}{r}@{}}
\hline
Dataset  & \multicolumn{1}{l|}{GM} & 
\multicolumn{1}{p{2cm}|}{\centering {BOP of the \newline last block}} & \multicolumn{1}{p{2cm}|}{\centering {BOP of the \newlinethree last blocks}} & \multicolumn{1}{p{2cm}|}{\centering {BOP of the \newline ten last blocks}} &\multicolumn{1}{p{2cm}|}{\centering {GM + BOP of \newline the  last block}} & \multicolumn{1}{p{2cm}|}{\centering {GM + BOP of \newline the  three last blocks}} & \multicolumn{1}{p{2cm}}{\centering {GM +BOP of \newline  the ten last block}} \\ \hline
CIFAR10    &\multicolumn{1}{c|}{96.94}&\multicolumn{1}{c|}{97.84}&\multicolumn{1}{c|}{98.28}&\multicolumn{1}{c|}{97.23}&\multicolumn{1}{c|}{ 98.37}&\multicolumn{1}{c|}{98.47}&\multicolumn{1}{c}{98.24}\\ \cline{1-1}
CIFAR100   &\multicolumn{1}{c|}{96.13}&\multicolumn{1}{c|}{93.59}&\multicolumn{1}{c|}{96.38}&\multicolumn{1}{c|}{ 97.35}&\multicolumn{1}{c|}{97.76}&\multicolumn{1}{c|}{97.90}&\multicolumn{1}{c}{98.07}&\\ \cline{1-1}
FMNIST     &\multicolumn{1}{c|}{94.74}&\multicolumn{1}{c|}{92.19}&\multicolumn{1}{c|}{93.65}&\multicolumn{1}{c|}{94.53}&\multicolumn{1}{c|}{ 94.76}&\multicolumn{1}{c|}{\textbf{94.50}}&\multicolumn{1}{c}{94.86}&\\ \cline{1-1}
CatsVsDogs &\multicolumn{1}{c|}{96.06}&\multicolumn{1}{c|}{97.80}&\multicolumn{1}{c|}{98.61}&\multicolumn{1}{c|}{96.76}&\multicolumn{1}{c|}{ 97.72}&\multicolumn{1}{c|}{98.31}&\multicolumn{1}{c}{\textbf{97.55}}\\ \cline{1-1}
DIOR &\multicolumn{1}{c|}{86.01}&\multicolumn{1}{c|}{85.68}&\multicolumn{1}{c|}{88.87}&\multicolumn{1}{c|}{95.21}&\multicolumn{1}{c|}{ 86.29}&\multicolumn{1}{c|}{86.51}&\multicolumn{1}{c}{\textbf{87.66}}&\\ 
\hline
\end{tabular*}
\caption{AUROC scores of the unimodal setting, using different blocks for the Block outputs prediction module}
\label{table:unimodal-aux}
\end{table*}


==> latex/tables/unimodal_transposed.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Dataset  &
\multicolumn{1}{c|}{CIFAR10} &
\multicolumn{1}{c|}{CIFAR100} &
\multicolumn{1}{c|}{FMNIST} &
\multicolumn{1}{c|}{CatsVsDogs} &
\multicolumn{1}{c|}{DIOR} \\
\hline
OC-SVM    &
\multicolumn{1}{c|}{64.7} &
\multicolumn{1}{c|}{62.6} &
\multicolumn{1}{c|}{92.8} &
\multicolumn{1}{c|}{ 51.7} &
\multicolumn{1}{c|}{70.7**} & 
\cline{1-1}
DeepSVDD   &
\multicolumn{1}{c|}{64.8} &
\multicolumn{1}{c|}{67.0} &
\multicolumn{1}{c|}{84.8} &
\multicolumn{1}{c|}{50.5} &
\multicolumn{1}{c|}{70.0*} &
\cline{1-1}
MHRot     &
\multicolumn{1}{c|}{90.1} &
\multicolumn{1}{c|}{80.1} &
\multicolumn{1}{c|}{93.2} &
\multicolumn{1}{c|}{86.0} &
\multicolumn{1}{c|}{73.3*} &
\cline{1-1}
CSI &
\multicolumn{1}{c|}{94.3} &
\multicolumn{1}{c|}{89.6} &
\multicolumn{1}{c|}{-} &
\multicolumn{1}{c|}{86.3*} &
\multicolumn{1}{c|}{78.5*} &
\cline{1-1}
DN2 &
\multicolumn{1}{c|}{92.5} &
\multicolumn{1}{c|}{94.1} &
\multicolumn{1}{c|}{94.5} &
\multicolumn{1}{c|}{96.0} &
\multicolumn{1}{c|}{92.2} & 
\cline{1-1}
PANDA &
\multicolumn{1}{c|}{96.2} &
\multicolumn{1}{c|}{94.1} &
\multicolumn{1}{c|}{\textbf{95.6}} &
\multicolumn{1}{c|}{97.6} &
\multicolumn{1}{c|}{\underline{94.3}} &
\cline{1-1}
MSAD &
\multicolumn{1}{c|}{97.5} &
\multicolumn{1}{c|}{\underline{96.5}} &
\multicolumn{1}{c|}{94.21} &
\multicolumn{1}{c|}{\textbf{99.4}} &
\multicolumn{1}{c|}{\textbf{97.2}} &
\cline{1-1}
GM &
\multicolumn{1}{c|}{96.94} &
\multicolumn{1}{c|}{96.13} &
\multicolumn{1}{c|}{94.74} &
\multicolumn{1}{c|}{96.06} &
\multicolumn{1}{c|}{86.01} &
\cline{1-1}
BoP &
\multicolumn{1}{c|}{\underline{98.28}} &
\multicolumn{1}{c|}{96.38} &
\multicolumn{1}{c|}{93.65} &
\multicolumn{1}{c|}{\underline{98.61}} &
\multicolumn{1}{c|}{88.87} &
\cline{1-1}
GM+BoP &
\multicolumn{1}{c|}{\textbf{98.47}} &
\multicolumn{1}{c|}{\textbf{97.90}} &
\multicolumn{1}{c|}{\underline{94.50}} &
\multicolumn{1}{c|}{98.31} &
\multicolumn{1}{c|}{86.51} &
\hline
\end{tabular}
\caption{{\bf AUROC scores of the unimodal setting.} We compare our three variants of our method (BoP only, GM only, and GM+BoP) against the alternative. We outperform all methods on both cifar10 and cifar100, and come in second on both the CatsVsDogs and FMNIST datasets.}
\label{table:unimodal}
\end{table}


==> latex/tables/whiten_var.tex <==
\begin{table*}
\begin{subtable}[l]{0.5\textwidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
 \thead{Explained \\ Variance} & Pre-Trained & Full \\
\hline
 $85\%$ & 96.85 & 98.11  \\
\hline 
 $90\%$ & 97.81 & 98.31 \\
\hline
 $95\%$ & 98.11 & 98.33 \\
\hline
\end{tabular}
\subcaption{Cifar10}
\end{subtable}
\begin{subtable}[c]{0.5\textwidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
 \thead{Explained \\ Variance}  & Pre-Trained & Full\\
\hline
 $85\%$ & 81.46 & 94.43  \\
\hline 
 $90\%$ & 81.06 & 94.32 \\
\hline 
 $95\%$ & 81.45 & 94.21 \\
\hline 
\end{tabular}
\subcaption{Wheather Recognition}
\end{subtable}
\caption{{\bf Sensitivity of Whitening hyper-parameter:} We whiten and reduce the dimensionality of the pre-defined features by keeping $90\%$ of the energy. In this experiment, we show the result of using either $85\%$ or $95\%$ of the energy on two different datasets. The left column, in each table, shows the performance of only the pre-trained features. The right column shows the performance of the full algorithm (pre-trained + fine-tuned features). As can be seen, the algorithm is not sensitive to this hyper-parameter.}
\label{table:whitening_var}
\end{table*}
